SelfHeal: Empirical Fix Pattern Analysis and Bug Repair in LLM Agents

Large Language Models (LLMs) have transformed software development and AI applications. While LLMs are designed for text processing, LLM agents extend this capability by enabling autonomous actions, tool use, and multi-step task completion. As this field grows, developers face new challenges in debugging these complex systems. To address this challenge, we present the first empirical study on bug fix patterns in LLM agents. We study buggy posts and code snippets from three platforms: Stack Overflow, GitHub, and HuggingFace Forums. We examine their fix patterns, the components where fixes are applied, and the programming languages and frameworks involved. Furthermore, we introduce AgentDefect, the first benchmark dataset for bugs in LLM agents. The dataset contains 37 runtime buggy instances along with fixed code and test files. Finally, we present SelfHeal, a multi-agent system designed to fix bugs in LLM agents. The system leverages two independent ReAct agents: the fix agent and the critic agent. These agents use tools that provide both internal knowledge (fix rules) and external knowledge (web search) to propose and validate fixes. Our evaluation shows that SelfHeal with Gemini 3 Pro as the backbone LLM outperforms both baseline and state-of-the-art approaches by a significant margin.

==> PatternTable.tex <==
\begin{table}[]
\caption{Fix Pattern Description}
\label{tab:fix-pattern-definition}
\begin{tabular}{|p{0.2\linewidth}|p{0.8\linewidth}|}
\hline
\textbf{Fix Pattern Name} & \textbf{Description} \\ \hline
Add New Attribute & Add new parameter value in the function call; either the default value was used or a required parameter was not passed. \\ \hline
Remove Attribute & Remove a parameter value to call the function with the default value. \\ \hline
Addition of Precondition Check & Add an if-else block before a specific code segment. \\ \hline
Change Version & Change the version of a specific library. \\ \hline
Install Library & Install a specific library. \\ \hline
Addition of Operations & Add a missing code block (e.g., ingestion stage for a RAG system). \\ \hline
Removal of Operations & Remove a specific code operation. \\ \hline
Change Data Type & Function is called with an incorrect data type. \\ \hline
Change Prompt & Incorrect prompt structure or input format. \\ \hline
Fix Syntax & Syntactic errors. \\ \hline
Change Reference & Incorrectly imported function or module. \\ \hline
Use Different Module & The used module is not compatible with the task. \\ \hline
Change External Resources & Issues related to environment, API, or external dependencies. \\ \hline
Change Function & Incorrect function used for a task. \\ \hline
Add Exception Handling & Add a try/except block. \\ \hline
Fix Attribute Name & Incorrect attribute or parameter name. \\ \hline
Change Parameter Value & Parameter type is correct but the value is incorrect. \\ \hline
Change Input Data & External input data is corrupted. \\ \hline
Add Input Data & System invoked without providing required input data. \\ \hline
Use Different Model & Use a different LLM. \\ \hline
Change Parameter Order & Incorrect parameter order in a function call. \\ \hline
Move Code to Different Scope & Code written in an incorrect scope. \\ \hline
Fix Data Access & Incorrect access to output data. \\ \hline
\end{tabular}
\end{table}

